On Using Stack Overflow Comment-Edit Pairs to recommend code maintenance changes

Code maintenance data sets typically consist of a before and after version of the code that contains the improvement or fix. Such data sets are important for software engineering support tools related to code maintenance, such as program repair, code recommender systems, or Application Programming Interface (API) misuse detection. Most of the current data sets are constructed from mining commit history in version-control systems or issues in issue-tracking systems. In this paper, we investigate whether Stack Overflow can be used as an additional data source. Comments on Stack Overflow provide an effective way for developers to point out problems with existing answers, alternative solutions, or pitfalls. In this paper, we mine comment-edit pairs from Stack Overflow and investigate their potential usefulness. These pairs have the added benefit of having concrete descriptions of why the change is needed as well as potentially having less tangled changes to deal with. We first design a technique to extract related comment-edit pairs and then investigate the nature of these pairs. We find that the majority of comment-edit pairs are not tangled, but only 27% of the studied pairs are potentially useful for the above applications. We categorize the types of mined pairs and find that the highest ratio of useful pairs come from categories Correction, Obsolete, Flaw, and Extension. To demonstrate the effectiveness of our extracted pairs, we submitted 15 pull requests on GitHub, 10 of which have been accepted to widely used repositories such as Apache Beam and nltk. Our work is the first to investigate Stack Overflow comment-edit pairs and opens the door for future work in this direction. Based on our findings and observations, we provide concrete suggestions on how to potentially identify a larger set of useful comment-edit pairs, which can also be facilitated by our shared data.

==> sections/pair-nature.tex <==
\section{Analyzing Comment-Edit Pairs}

After building and evaluating a program to find comment-edit pairs, our goal is to analyze a collection of these pairs to understand their nature.
We first run our matching program on the data from all the five tags we focus on.
Table~\ref{tab:LanguageStatistics} shows the descriptive statistics for this data, as well as the number of comment-edit pairs detected by our tool.

\begin{table}[t!]
\centering
\caption{Statistics on the language tags}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Language}   & 
\multicolumn{1}{l}{\textbf{Answers}} & 
\multicolumn{1}{l}{\textbf{Edits}} & 
\multicolumn{1}{l}{\textbf{Comments}} & 
\multicolumn{1}{m{2cm}}{\textbf{Comment-edit pairs}} \\
\midrule
\textbf{Java}       & 2,586,447 & 895,737  & 2,321,296 & 51,358 \\
\textbf{Javascript} & 2,924,662 & 1,281,433 & 3,571,622 & 65,373 \\
\textbf{Android}    & 1,722,580  & 490,565  & 1,668,634 & 34,596 \\
\textbf{Python}     & 1,785,914 & 903,159  & 2,060,513 & 44,551 \\
\textbf{Php}        & 2,099,914 & 751,612  & 2,508,003 & 52,521 \\
\bottomrule
\end{tabular}
\label{tab:LanguageStatistics}
\end{table}

\subsection{Determining comment-edit pairs to categorize} 

To accurately categorize comment-edit pairs, we need a set of confirmed pairs so that we can have confidence in our categorization.
Since it is not feasible to manually validate close to 250,000 pairs, we take a statistically representative sample for each tag.
For a confidence level of 95\% with a 5\% confidence interval we calculate the sample size of comment-edit pairs we need to be 382 pairs for each tag.
We randomly select the 382 pairs we analyze for each tag.

\input{sections/table-categories.tex}

%The equation for calculating sample size is defined in Equation~\ref{SampleSizeCalculation}. 
%Where $Z$ is the Z value determined by the confidence level, $p$ is the percentage picking a choice, and $c$ is the confidence interval.
%\begin{equation}
%ss = \frac{Z^2 * (p) * (1 - p)}{c^2}
%\label{SampleSizeCalculation}
%\end{equation}
%According to Equation~\ref{SampleSizeCalculation} we calculated that to calculate the general precision of the matched pairs we need to manually analyze ~382 comment-edit pairs per language. 

The two authors then separately analyze all \checkNum{1910} comment-edit pairs, with the goal of confirming that the identified comment is what caused the corresponding edit in the pair.
Thus, each comment-edit pair was labeled with either 0 (comment is not the cause for the edit) or 1 (comment is the cause for the edit).
After the separate labeling process, both authors discussed any disagreements and resolved conflicts.
%Each author manually analyzed the comment-edit pairs individually and compared their results afterward.
%The criteria to determine the validity of the pair is different than the criteria used for the ground truth set.
%The criteria used for the ground truth was to look at all comments and edits of an answer and the matched pairs returned by the program and determine if the comment in the pair was \textbf{related} to the edit in the pair. 
%For determining the general precision the criteria was not whether or not the comment was related to the edit in a pair, but if the comment was the \textbf{cause} of the edit.
%This criteria makes the manual analysis of the general precision easier than the analysis of the ground truth as there only needs to be a yes/no confirmation of whether the comment in the comment-edit pair caused the edit.
%After each author analyzed the comment-edit pairs, the results were combined into one spreadsheet and the authors then discussed the disagreements they had.
%Most of the disputes were when one author thought the matched comment and edit were unrelated but the other disagreed.
%This is usually the case when the edit is fairly large and it seems like the related code in the comment was only by coincidence.
Our inter-rater agreement, calculated using Cohen's Kappa Score~\cite{viera2005understanding} was substantial at \checkNum{0.84} for Java and \checkNum{0.71} for JavaScript.
This manual validation also allows us to calculate the precision of the automated matching strategy on a larger statistically representative sample.
We find that the precision for Java is \checkNum{52.36\%} and \checkNum{52.09\%} for JavaScript.
This is lower than what we previously obtained in our ground truth, which we attribute to two reasons.
The first is the different sample which contains pairs from a larger sample of diverse answers.
The second is that both authors erred on the side of caution when evaluating the comment-edit pairs and when resolving disputes.
Any uncertainty about whether a comment actually caused an edit was marked as a no, since any imprecision in the resulting set of confirmed comment-edit pairs would result in misleading categorizations in the next step.
This process resulted in a total of \checkNum{399} verified comment-edit pairs, \checkNum{200} from Java and \checkNum{199} from Javascript, which we use in the next step.


\subsection{Categorizing comment-edit pairs} 
During the manual validation step above, we also wrote a short description of the situation that resulted in the edit. Examples of our descriptions include \textit{``commenter points out problematic API method (can result in exception) and editor edits the answer to include that warning''}  or \textit{``commenter does not understand how the output is being printed in the code and Editor updates with more explanation and a fleshed out example.''}
We categorize these descriptions for the 399 verified comment-edit pairs using open coding, specifically card sorting~\cite{ZIMMERMANN2016137}. 
Our card sorting process resulted in 16 labels, which we grouped into 5 categories.
Table~\ref{tab:categories} shows these categories, the sub-categories (i.e., label) under each category, and the number of corresponding pairs.
We also provide an example comment to illustrate each sub-category
We now discuss these categories.



Table~\ref{tab:categories} shows that 26\% of the 399 pairs we analyzed (=105 pairs) involved reports on errors, exceptions, or incorrect/unexpected behavior.
In these cases, the commenter typically reports the failure and the editor changes the posted code to solve the problem.
The next highest category is insufficient answer (102/399 = 26\%). 
Here, the posted answer is typically wrong or incomplete in some way.
This could include simple typos or changes required to the code to make it catch all corner cases.
Help requests were also common in the analyzed comment-edit pairs (86/399 = 22\%).
Help requests include clarifications on the posted answer and explicit requests for additional examples.
In 61 (15\%) of the pairs we analyzed, the answer was correct but the commenter was providing suggestions for potential improvements, such as mentioning an alternative API that can be used or improving non-functional properties such as memory usage. 
Additional improvements included making the solution more general rather than, for example, hard-coding things specific to the original poster's question or simple code style improvements such as better variable names. 
This is interesting since it suggests that Stack Overflow may be more promising for finding code improvement and non-functional changes as opposed to, for example, mining historical commits~\cite{Radu:2019}.
Finally, we also find 45 pairs (11\%) where the comments are mainly clarifying the needed requirements or the setup.
It is worth noting that many of these included updates to the original question, as indicated in the comment.
It is not surprising to see such types of comments, given that reproducing a problem and finding a solution to it requires lots of information about the intended behavior and the setup used, but this also suggests that work on finding required question clarifications (e.g.,~\cite{RaoDaumClarificationQuestions}) may need to include answer comments in addition to question comments




==> sections/pair-stats.tex <==
\subsection{Quantitative Analysis of Comment-Edit Pairs}

The previous qualitative analysis revealed the categories of comments that result in answer edits.
However, it does not provide us enough information about the relationship between the users behind the comments and updates.
For example, is the person making the comment usually the original poster (OP) of the question or do other community members provide comments?
Is the user who made the edit usually the one who originally posted the answer?
Another interesting aspect is the score of the answer.
Does a confirmed edit-comment pair mean that the answer was ``bad'' (low score) in the first place, or do the posted comments that result in edit happen on highly scored answers, or at least can help already good answers become better?
To investigate all these questions, we quantitatively analyze the relationship between the OP (questioner), the answer poster (answerere), the answer editor (editor), and the commenter.
We also collect the scores of the confirmed comment-edit pairs, and the response time between each comment and its matched edit.
Table~\ref{tab:CategoryStats} shows the results of the 200 Java and 199 Javascript answers we analyzed.
We show the results per category, as well as the total across all pairs in each tag.

Our first observation is that the commenter and the editor are usually different.
This is probably due to the fact that a user editing an answer would directly make the edit first rather than make a comment and then edit the answer.
There were only a few cases where the commenter and editor were the same.
% AnswerId: 10270638
For example, in \post{10270638}, the commenter (Josh) points out two mistakes in the code.
The answerer (Manishearth) acknowledges the mistake, but asks Josh to perform the edit since they are on their phone.   
Apart from such rare cases, our results show that the commenter and editor are typically different and that the editor is typically the original author of the answer. 
This is most likely, because as the answer poster they have the most understanding of the answer than anyone else, which allows them to make the necessary edits.
There are only a few cases when a third party performs the edit (Answerer/Editor different), and this demonstrates the community aspect of Stack Overflow.

While in the majority of cases, the comment that resulted in the edit was posted by the original question poster (Questioner/Commenter same), it is interesting to see that in a total of 141 pairs (35\%) across both tags, the commenter was a third party.
This demonsrates another advantage of Stack Overflow where the posted answers are vetted by many developers world wide.
These developers can then spot problems or suggest better alternatives, which helps improve the overall quality of the posted code snippets.
Looking more closely at the statistics of the individual categories in Table~\ref{tab:CategoryStats}, we can see that the comments related to improvements and insufficient answers are more likely to be posted by someone other than the original question asker.
A Chi-Squared test does indeed show that there is a relationship between the category and whether the the commenter is the same as the questioner ($p = 0.00$).
We discuss the implications of this phenomenon in Section~\ref{sec:discussion}.
Similarly, we can see that the average response time to both these types of comments is much longer than the average response time for the other categories.
However, a non-paired Wilcoxon signed-rank test shows that this difference is not statistically significant.
We find that while this huge difference in mean values mainly comes from some outliers that skew the average, but the distributions are similar based on the statistical test.

%The majority of commenters that cause edits in an answer also appears to be the question asker.
%This could be clarifications on information that was not included in the question or that the answer was not sufficiently clear and the questioner asked some follow-up question that resulted in edits to the answer.

The average answer scores shown in Table~\ref{tab:CategoryStats} suggest that the answers that receive comments resulting in updates are not necessarily ones with a low score.
This aligns with previous findings that show that the number of comments an answer receives is not correlated with its score~\cite{AdajiEditComment}.
However, a Wilcoxon signed-rank test, with a Benjamini \& Hochberg (BH) p-value adjustment measure to account for multiple comparisons, shows that there are statistically significant differences in the answer score distribution between the various categories.
Specifically, we find that the Improvements category is statistically different from Error reporting ($p=0.01$), Help requests ($p=0.00$), and Requirements refinement ($p=0.00$).
Based on Table~\ref{tab:CategoryStats}, it seems that improvement comments and their resulting edits happen on average to answers with higher scores.

%\begin{table}[]
%\centering
%\caption{Quantitative analysis of the relationship between comments and edits}
%\begin{tabular}{lrr}
%\toprule
%\textbf{} & 
%\textbf{Java} & 
%\textbf{Javascript} \\
%\midrule
%\textbf{Commenter/Editor Same}          & 7    & 6    \\
%\textbf{Commenter/Editor Different}     & 193  & 193  \\
%\addlinespace
%\textbf{Answerer/Editor Same}           & 188  & 185  \\
%\textbf{Answerer/Editor Different}      & 12   & 14   \\
%\addlinespace
%\textbf{Questioner/Commenter Same}      & 130  & 128  \\
%\textbf{Questioner/Commenter Different} & 70   & 71   \\
%\addlinespace
%\textbf{Answer Score above 0}           & 197  & 197  \\
%\textbf{Answer Score below 0}           & 3    & 2    \\    
%\textbf{Average Answer Score}           & 13.9 & 16.1 \\   
%\addlinespace
%\textbf{Average Respone Time}           & 34 days & 26 days \\
% 
%\bottomrule                             
%\end{tabular}
%\label{GPStatistics}
%\end{table}


\begin{table*}[t!]
\centering
\caption{Quantitative analysis of the relationship between comments and edits by category}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
& 
\multicolumn{2}{c}{\textbf{{Error Reporting}}}
& \multicolumn{2}{c}{\textbf{Help requests}}                                                    
& \multicolumn{2}{c}{\textbf{Improvements}}                                                                                                   
& \multicolumn{2}{c}{\textbf{Insufficient Answer}}                                                   & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}l@{}}Requirements \\ Clarification\end{tabular}}}&
 \multicolumn{2}{c}{\textbf{All}}
\\
& 
\textbf{Java} & \textbf{JS} & 
\textbf{Java} & \textbf{JS} & 
\textbf{Java} & \textbf{JS} & 
\textbf{Java} & \textbf{JS} & 
\textbf{Java} & \textbf{JS*} & 
\textbf{Java} & \textbf{JS} \\
\midrule
\textbf{Commenter/Editor Same} & 1 & 1 & 1 & 1 & 2 & 0 & 2 & 4 & 1 & 0 & 7 & 6\\
\textbf{Commenter/Editor Different} & 53 & 50 & 47 & 37 & 31 & 27 & 40 & 55 & 22 & 21 & 193 & 193 \\
\midrule
\textbf{Answerer/Editor Same} & 52 & 47 & 47 & 37 & 31 & 23 & 36 & 54 & 22 & 21 & 188 & 185\\
\textbf{Answerer/Editor Different} & 2 & 4 & 1 & 1 & 2   & 4 & 6  & 5 & 1 & 0 & 12 & 14\\
\midrule
\textbf{Questioner/Commenter Same} & 44 & 43 & 46 & 33 & 2 & 3 & 15 & 29 & 23 & 19 & 130 & 128\\
\textbf{Questioner/Commenter Different} & 10 & 8 & 2 & 5 & 31 & 24 & 27 & 30 & 0 & 2 &70 & 71 \\
\midrule
%\textbf{Answer Score $>= 0$} & 53 & 51 & 47 & 38 & 33 & 26 & 41 & 58 & 23 & 21 & 197 & 197\\
%\textbf{Answer Score $< 0$} & 1 & 0 & 1 & 0 & 0 & 1 & 1 & 1 & 0 & 0 & 3 & 2\\
\textbf{Average Answer Score} & 3 & 2 & 2 & 6 & 31 & 62 & 34 & 20 & 1  & 1 & 14 & 16 \\
\midrule
\textbf{Average Response Time}         & \begin{tabular}[c]{@{}l@{}}0d \\ 05:02h\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0d\\ 07:59h\end{tabular} & \begin{tabular}[c]{@{}l@{}}0d \\ 03:37h\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0d\\ 03:33h\end{tabular} & \begin{tabular}[c]{@{}l@{}}25d\\ 07:23h\end{tabular} & \begin{tabular}[c]{@{}l@{}}62d\\ 11:36h\end{tabular} & \begin{tabular}[c]{@{}l@{}}142d\\ 15:08h\end{tabular}      & \begin{tabular}[c]{@{}l@{}}44d\\ 10:33h\end{tabular} & \begin{tabular}[c]{@{}l@{}}0d\\ 17:57h\end{tabular}                & \begin{tabular}[c]{@{}l@{}}0d\\ 04:23h\end{tabular} & 34d & 26d
 \\

\bottomrule
\end{tabular}
\begin{flushright}
\textbf{* One outlier with response time $>$1000 days was removed}
\end{flushright}
\label{tab:CategoryStats}
\end{table*}

%\begin{figure}[t!]
%\centering
%  \includegraphics[width=0.4\textwidth]{images/AnswerDistribution.pdf}
%  \caption{Distribution of answer scores in the confirmed 399 comment-edit pairs}
%  \label{fig:GPAnswerDist}
%\end{figure}


==> sections/table-categories.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}


\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\begin{table*}[ht!]
\centering
\caption{Categories of 399 analyzed comment-edit pairs}
\label{tab:categories}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cp{2cm}p{3cm}p{8.5cm}rrr@{}}
\toprule
\textbf{Category}                        & \textbf{Description}                                                                & \textbf{Sub-category}               & \textbf{Example comment}                                                                                                                                                                                                                                                                                                                                                                        & \textbf{Java} & \textbf{Javascript} & \textbf{Total} \\ \midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Error reporting}}}
%\multirow{3}{*}{\textit{Error reporting}}     
& \multirow{3}{2cm}{Reports of observed failures}                                                        & Errors or exceptions                  & \post{44470955}: ``The console says: "Uncaught ReferenceError: Invalid left-hand side in assignment" in the line of "this = x.concat..." ''                                                                                                                                                                                                                                                   & 36                  & 28                        & 64                   \\
                                             &                                                                                     & Unexpected or different behavior                   & \post{37339594}: ``It isnt working.. it is considering productObject as one whole string not each part of it as object...''                                                                                                                                                                                                                                                                   & 18                  & 23                       & 41                   \\
%                                             &                                                                                     & Still doesn't solve the problem       & \post{37776174}: ``ok it reads from database now. But ...still without style. :S i also tried to edit \texttt{\$('\#output').empty().append(\_ul);} to [..]''                                                                                                                                                                                                                                 & 3                   & 12                        & 15                   \\
\cmidrule{4-7}
                         &                                                                                     &                                       &                                                                                                                                                                                                                                                                                                                                                                                               Total category count & 54                  & 51                        & 105                  \\
%%%%%%%
\midrule
%%%%%%%
\multirow{2}{*}{\rotatebox[origin=c]{90}{}}
%\multirow{8}{*}{\textit{Insufficient answer}} 
& \multirow{7}{2cm}{The answer requires corrections to address the question \& work correctly}           &    Incorrect or wrong logic              & \post{55688314}: ``try \texttt{str.replace(/s*his/g, (p)=>`<span>\${p}</span>`)} and you will see that your solution does not include the spaces captured''                                                                                                                                                                                                                                    & 13                  & 14                       & 27                   \\


                                             &                                                                                     & Exact code changes that worked        & \post{28880306}: `[..] I've decided to:first set var \_\_coordinates = [], and then check for coordinates.sort().toString() != \_\_coordinates.sort().toString() . This seems to work. Olivier, I already marked your answer as correct, but if you could edit your answer to use one of these that work ...''                                                                                   & 6                   & 12                        & 18                   \\
%                                             &                                                                                     & Code review like content              & \post{32170233}: ``You should declare \$age before you use it''                                                                                                                                                                                                                                                                                                                                & 3                   & 9                         & 12                   \\
 
 \multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{Insufficient answer}}}& &Incorrect syntax                      & \post{49363980}: ``You meant \texttt{\$(evt.target).parent().css…} don't you ?''                                                                                                                                                                                                                                                                                                               & 4                   & 12                         & 16                    \\
                                             
                                                                                          &                                                                                     & Typos                                 & \post{49060906}: ``It worked. Minor typo error in your code. It should be insertMany instead of insertAll. Thanks a lot!!''                                                                                                                                                                                                                                                                   & 7                   & 8                         & 15                   \\
                                             
& & Alternative correct solution or API provided & \post{37762134}: You should instead use \texttt{get(new GenericType<List<Phase1Bean>>(){});}. What you are doing will give you a raw List, which will be populated with LinkedHashMaps, instead of Phase1Beans                                                                                                                                                                                & 8                   & 6                         & 14                    \\                                             
                                             &                                                                                     & Missing corner cases or requirements  & \post{18493467}: ``I could be wrong but I don't think this solution would be able to detect whether there is more than one of the same element in a List....''                                                                                                                                                                                                                                & 4                   & 8                         & 12                   \\

\cmidrule{4-7}                                             
                          &                                                                                     &                                       &                                                                                                                                                                                                                                                                                                                                                                                               Total category count& 42                  & 60                        & 102                   \\

%%%%%%%
\midrule
%%%%%%%

%\multirow{4}{*}{\textit{Help requests}}       
& \multirow{4}{2cm}{Help is needed to understand or use the provided code/solution}     &                                                                           Request for examples \& how to use provided code              & \post{30511497}: ``... which item do I need to pass to both the View v and MotionEvent event parameter of the onTouch method? I have also written public boolean onTouch(View v, MotionEvent event){return true;}''                                                                                                                                                                           & 21                  & 16                        & 37                   \\

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Help requests}}}& & Clarifications about posted answer    & \post{53967874}: `why [does] the JsonAdapter extend XmlAdapter? what has xml got to do with it?''                                                                                                                                                                                                                                                                                             & 20                  & 7                         & 27                   \\
%                                             &                                                                                     & Request for more explicit examples    & \post{42469760}: ``I'm asking [..] for an example of \texttt{Executors.newSingleThreadExecutor()}''                                                                                                                                                                                                                                                                                           & 2                   & 1                         & 3                    \\
                                             &                                                                                     & New/extra/follow-up questions         & \post{52454084}: ``I removed the .link(roomNames) so that it wont redirect me to another page. How do I show the data of a classroom when I click it?''                                                                                                                                                                                                                                       & 7                   & 15                        & 22                   \\
\cmidrule{4-7}
                          &                                                                                     &                                       &                                                                                                                                                                                                                                                                                                                                                                                               Total category count& 48                  & 38                        & 86                   \\

%%%%%%
\midrule
%%%%%%%




%\multirow{5}{*}{\textit{Improvements}}        
&\multirow{7}{2cm}{Answer is correct, but comment provides improvements}               &   Simplicity \& ease of use              & \post{22801381}: ``Why not just write \texttt{B\_arrayList.retainAll(A\_arraylist);}? Don't reinvent wheels!''                                                                                                                                                                                                                                                                                  & 15                  & 12                        & 27                   \\

                                              &                                                                                     & Best practices \& code style           & \post{18787645}: ``I have used this a few times and think there are two tweaks that make it better for the real world application. 1) lowercase the L in \texttt{multiLog} so the function name is multilog. I have got confused a couple of times. 2) replace the \texttt{console.log(toLog[i]);} to \texttt{console.log(toLog[i] + ' =>');} It just makes it a bit clearer when debugging'' & 7                   & 4                         & 11                   \\


\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Improvements}}}&& Generalizability                      & \post{37992391}: ``I would change the function slightly and call it addText(String text, String hexColor) and pass in the string to be colored and pass in a string representing the hex color. Now you can color text any color you want.''                                                                                                                                                  & 4                   & 5                         & 9                    \\
                                              &                                                                                     & Redundant code                        & \post{14499028}: ``Don't need to call \texttt{toString();} on a \texttt{String.}''                                                                                                                                                                                                                                                                                                            & 2                   & 4                         & 6                    \\

                                              &                                                                                     & Non-functional properties             & \post{37992391}: ``You don't need to pass \texttt{list.size()}, this will just create an overhead of a bigger temporary array created that will be discarded right away. I could just be \texttt{String[] arr = list.toArray(new String[] {});}'                                                                                                                                              & 4                   & 0                         & 4                    \\


                                             &                                                                                     & Possible alternative APIs                    & \post{13955260}: ``a great addition to your answer would be: \texttt{console.log(Object.prototype === me.\_\_proto\_\_);'}'                                                                                                                                                                                                                                                                       & 1                   & 3                         & 4                    \\
\cmidrule{4-7}
                         &                                                                                     &                         &                                                                                                                                                                                                                                                                                                                                                                                               Total category count               & 33                  & 28                        & 61                   \\
                         %%%%%%%
\midrule
%%%%%%%

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Req. Refinement}}}
%\textit{Requirements Clarification}           
& Provides additional information about requirements                                           & Requirements refinement            & \post{26051940}: ``Unfortunately I am working in a system where the jQuery listener is already defined, and I'm trying to write vanilla javascript that can utilize it. So unfortunately this does not help, but thanks anyway!''                                                                                                                                                             & 23                  & 22                        & 45                   \\
\cmidrule{4-7}
                          &                                                                                     &                                       &                                                                                                                                                                                                                                                                                                                                                                                               Total category count& 23                  & 22                        & 45                   \\

\bottomrule
\end{tabular}%
}
\end{table*}

